MGTCOM: Community Detection in Multimodal Graphs

Community detection is the task of discovering groups of nodes sharing similar patterns within a network. With recent advancements in deep learning, methods utilizing graph representation learning and deep clustering have shown great results in community detection. However, these methods often rely on the topology of networks (i) ignoring important features such as network heterogeneity, temporality, multimodality, and other possibly relevant features. Besides, (ii) the number of communities is not known a priori and is often left to model selection. In addition, (iii) in multimodal networks all nodes are assumed to be symmetrical in their features; while true for homogeneous networks, most of the real-world networks are heterogeneous where feature availability often varies. In this paper, we propose a novel framework (named MGTCOM) that overcomes the above challenges (i)--(iii). MGTCOM identifies communities through multimodal feature learning by leveraging a new sampling technique for unsupervised learning of temporal embeddings. Importantly, MGTCOM is an end-to-end framework optimizing network embeddings, communities, and the number of communities in tandem. In order to assess its performance, we carried out an extensive evaluation on a number of multimodal networks. We found out that our method is competitive against state-of-the-art and performs well in inductive inference.

==> figs/abl/img_abl_beta.tex <==
\begin{figure*}[ht!]
\centering

\includegraphics[width=\textwidth]{resources/figs/abl_beta_topo.pdf}

\caption{
Performance of $MGTCOM$ model while varying topological loss weight parameter $\beta^{\mathcal{T}}$ under $1 = \beta^{\mathcal{E}}$ + $\beta^{\mathcal{T}}$ contraint.
}
\label{fig:abl_beta}
\end{figure*}

==> figs/abl/img_abl_embed_ratio.tex <==
\begin{figure}[ht]
\centering

\includegraphics[width=0.8\columnwidth]{resources/figs/embed_ratio.pdf}

\caption{
Performance results for topological $MGTCOM^{\mathcal{E}}$ and temporal $MGTCOM^{\mathcal{T}}$ models on various tasks where the ratio of auxiliary embedded nodes varies.
}
\label{fig:abl_embed_ratio}
\end{figure}

==> figs/abl/img_abl_k.tex <==
\begin{figure}[ht]
\centering

\subfigure[]{
\includegraphics[width=0.35\textwidth]{resources/figs/abl_initk_k.pdf}
}
\subfigure[]{
\includegraphics[width=0.35\textwidth]{resources/figs/abl_initk_dbi.pdf}
}

\caption{
(a) and (b): Cluster count progression during DPMM clustering given an initial cluster count (init $K$). The clustering is done on pre-trained $MGTCOM$ embeddings for the DBLP dataset.
}
\label{fig:ablation_k}
\end{figure}

==> figs/abl/img_abl_meta.tex <==
\begin{figure*}[ht]
\centering

\includegraphics[width=0.8\textwidth]{resources/figs/abl_meta.pdf}

\caption{
Performance results for (a) topological $MGTCOM^{\mathcal{E}}$ and (b) temporal $MGTCOM^{\mathcal{T}}$ models, on prediction tasks for heterogeneous and homogeneous variants of the DBLP dataset.
To determine the importance of meta-topological attention we vary the convolutional layers HGT and GraphSAGE (which is adopted for heterogeneous graphs).
}
\label{fig:ablation_meta}
\end{figure*}

==> figs/alg_temporw.tex <==
\begin{algorithm}[!t]
    \small
    \caption{Temporal Random Walk}\label{alg:tempo_rw}
    \SetKwFunction{algo}{BallroomWalk}
    \SetKwFunction{proc}{TemporalRW}
    \SetKw{KwGoTo}{go to}
    
    \setcounter{AlgoLine}{0}
    \SetKwProg{myproc}{Procedure}{}{}
    \myproc{\proc{}}{
    \KwIn {
        center node $v$,
        temporal window $\omega^*$
    }
    \KwOut {
        Temporal random walk $P_l$
    }
        Initialize $P_l$ = $[]$\; 
        $(u, t_u) = (v, \varnothing)$\;
        \For {$i = 1$ \KwTo $l$} {
            $N(u) = \{w| 
                w \in \mathcal{V}, 
                (u, w) \in \mathcal{E},
                \tau(w) \cap \omega^* \neq \emptyset
            \}$\; \label{alg:trw:neighbors}
        
            \If (\tcc*[h]{Restart on dead end}){$N(u) = \emptyset$}{
                $(u, t_u) = (v, t_v)$\; \label{alg:trw:restart}
                \KwGoTo \ref{alg:trw:neighbors}\;
            }

            $w \sim N(u)$\; \label{alg:trw:sample}
            $t_u = \max \left\{ t_u, \min{ \tau(w)} \right\}$\;
            $u = w$\;

            $P_{l}.append((u, u_t))$\;
        }

        \KwRet $P_l$
    }
\end{algorithm}

==> figs/hyp/img_hyp_cluster.tex <==
\begin{figure}[]
\centering
\subfigure[]{
\includegraphics[width=0.21\textwidth]{resources/figs/cluster_alpha.pdf}
}
\subfigure[]{
\includegraphics[width=0.21\textwidth]{resources/figs/cluster_sigma_scale.pdf}
}
\subfigure[]{
\includegraphics[width=0.21\textwidth]{resources/figs/cluster_nu.pdf}
}
\subfigure[]{
\includegraphics[width=0.21\textwidth]{resources/figs/cluster_kappa.pdf}
}
\caption{
    Sensitivity of the resulting cluster count $K$ on the DPMM prior parameters (a) $\alpha$ the cluster concentration parameter, (b) the $\sigma$ scale parameter influencing the covariance of prior, (c) $\nu$ the degrees of freedom parameter for the Wishart prior distribution, and (d) $\kappa$ the concentration parameter of the Wishart prior distribution.
}
\label{fig:hyp_cluster}
\end{figure}

==> figs/hyp/img_hyp_neigh.tex <==
\begin{figure}[]
\centering

\includegraphics[width=\columnwidth]{resources/figs/tune_topo_neigh.pdf}

\caption{
Performance of $MGTCOM^{\mathcal{E}}$ model with varying convolution layers. 
We vary the architecture by switching between Heterogeneous Graph Transformer (HGT) and Heterogenous GraphSAGE convolutional layers.
Similarly, we also modify the neighborhood size of each node within the two-layer convolution setup. 
Format $(x, y)$ represents the number of neighbors per node in the first ($x$) and second ($y$) layer respectively.
}
\label{fig:hyp_neigh}
\end{figure}

==> figs/hyp/img_hyp_rep_margin.tex <==
\begin{figure*}[ht!]
\centering
\subfigure[]{
\includegraphics[width=0.32\textwidth]{resources/figs/tune_topo_reprdim.pdf}
}
\subfigure[]{
\includegraphics[width=0.32\textwidth]{resources/figs/tune_topo_margin.pdf}
}
\subfigure[]{
\includegraphics[width=0.32\textwidth]{resources/figs/tune_topo_activation.pdf}
}
\caption{
Performance of $MGTCOM^{\mathcal{E}}$ model with varying (a) representation dimension $d$, (b) the margin ($\Delta$) parameter for the hinge loss, and (c) activation function.
}
\label{fig:hyp_rw_repr}
\end{figure*}    

==> figs/hyp/img_hyp_rw_tempo.tex <==
\begin{figure}[ht!]
\centering
\subfigure[]{
\includegraphics[width=0.35\textwidth]{resources/figs/tune_tempo_rw_ctx.pdf}
}\quad
\subfigure[]{
\includegraphics[width=0.35\textwidth]{resources/figs/tune_tempo_rw_nwalks.pdf}
}\quad
\caption{
Performance of $MGTCOM^{\mathcal{T}}$ model with varying (a) random walks length $l$ and (b) number of random walks per node $n$.
}
\label{fig:hyp_rw_tempo}
\end{figure}    

==> figs/hyp/img_hyp_rw_topo.tex <==
\begin{figure*}[ht!]
\centering
\subfigure[]{
\includegraphics[width=0.3\textwidth]{resources/figs/tune_topo_rw_ctx.pdf}
}
\subfigure[]{
\includegraphics[width=0.3\textwidth]{resources/figs/tune_topo_rw_nwalks.pdf}
}
\subfigure[]{
\includegraphics[width=0.3\textwidth]{resources/figs/tune_topo_rw_q.pdf}
}
\caption{
Performance of $MGTCOM^{\mathcal{E}}$ model with varying (a) random walks length $l$, (b) number of random walks per node $n$, and (c) the exploration trade-off parameter $q$.
}
\label{fig:hyp_rw_topo}
\end{figure*}    

==> figs/img_em.tex <==
\begin{figure}[t!]
\centering
\subfigure[]{
% \includegraphics[width=0.40\columnwidth]{resources/em/EM1.png}
\includegraphics[width=0.21\textwidth]{resources/em/EM1.png}
}\quad
\subfigure[]{
% \includegraphics[width=0.40\columnwidth]{resources/em/EM2.png}
\includegraphics[width=0.21\textwidth]{resources/em/EM2.png}
}\quad
\subfigure[]{
% \includegraphics[width=0.40\columnwidth]{resources/em/EM3.png}
\includegraphics[width=0.21\textwidth]{resources/em/EM3.png}
}\quad
\subfigure[]{
% \includegraphics[width=0.40\columnwidth]{resources/em/EM4.png}
\includegraphics[width=0.21\textwidth]{resources/em/EM4.png}
}\quad
\caption{
Visualization of Expectation-Maximization algorithm \cite{bishopPatternRecognitionMachine2006}.
(a) Clusters are randomly initialized. 
(b) Cluster centers are updated according to the initial assignment (M step).
(c), (d) Expectation and Maximization steps are repeated until convergence.
}
\label{fig:em}
\end{figure}    

==> figs/img_hgt.tex <==
\begin{figure}[!ht]
\centering
\includegraphics[width=\columnwidth]{resources/hgt.pdf}
\caption{
    Visualization of a Heterogeneous Graph Transformer Layer. Given target node $t$ and neighboring source nodes $s_1$ and $s_2$ by edges $e_1$ and $e_2$, mutual attention and messages are computed. Within aggregation step the messages are attended and combined with previous target node embedding $H^{(l-1)}_t$ resulting in the new embedding vector $H^{(l)}_t$
}
\label{fig:hgt}
\end{figure}    

==> figs/tab_config.tex <==
\begin{table}[t!]
\centering
\caption{
    Complete overview of used parameters for $MGTCOM$ and its variants for bench marking and tuning.
} \label{tab:config}
\begin{tabular}{lll}
\toprule
                       Config key &   Value \\
\midrule
                            loss &   HINGE \\
                    hinge\_margin &     0.1 \\
                          metric &    DOTP \\
                              lr &    0.02 \\
                        repr\_dim &      64 \\
                    lp\_max\_pairs &    5000 \\
    ballroom\_params/context\_size &      10 \\
 ballroom\_params/num\_neg\_samples &       1 \\
     ballroom\_params/walk\_length &      20 \\
  ballroom\_params/walks\_per\_node &      10 \\
         n2v\_params/context\_size &      10 \\
      n2v\_params/num\_neg\_samples &       1 \\
                    n2v\_params/p &       1 \\
                    n2v\_params/q &     0.5 \\
          n2v\_params/walk\_length &      20 \\
       n2v\_params/walks\_per\_node &      10 \\
                embed\_node\_ratio &     1.0 \\
                  conv\_num\_heads &       2 \\
                 conv\_num\_layers &       2 \\
                     num\_samples &  [3, 2] \\
                  sampler\_method &     HGT \\
                  split\_num\_test &     0.1 \\
                   split\_num\_val &     0.1 \\
                tempo\_hidden\_dim &      32 \\
                  tempo\_repr\_dim &      64 \\
                    tempo\_weight &     1.0 \\
                 topo\_hidden\_dim &      32 \\
                   topo\_repr\_dim &      64 \\
                     topo\_weight &     1.0 \\
                       use\_tempo &    True \\
                        use\_topo &    True \\
                         infer\_k &       3 \\
                     prior\_alpha &     1.0 \\
                     prior\_kappa &     1.0 \\
                        prior\_nu &      65 \\
                prior\_sigma\_scale &     0.1 \\
\bottomrule
\end{tabular}
\end{table}

==> figs/tab_inference.tex <==
\begin{table*}[t!]
\centering
\caption{
    Comparison of different model variants in the inference-based setting. 
    Graph nodes are split into three disjointed sets (train, validation, and test).
    The metrics are measured while the training to validation ratio is varied. 
    The test set is set to 10\% of the nodes and is kept constant.
}
\label{tab:results_inference}
% \resizebox{\textwidth}{!}{
    \begin{tabular}{ll|ccccccccc}
    \toprule
     \textbf{Model}                      & \textbf{\% Train} &            10\% &            20\% &            30\% &            40\% &            50\% &            60\% &            70\% &            80\% &            90\% \\ 
    \midrule
$MGTCOM$ 
                       & $LP_{ACC}$ &  0.686 &  0.728 &  0.774 &  0.755 &  0.780 &  0.833 &  0.861 &  0.887 &  0.872 \\
                       & $CF_{ACC}$ $L_y$ &  0.428 &  0.474 &  0.548 &  0.571 &  0.638 &  0.799 &  0.861 &  0.899 &  0.927 \\
                       & $CF_{ACC}$ $L_\mathcal{T}$ &  0.323 &  0.333 &  0.370 &  0.408 &  0.483 &  0.566 &  0.664 &  0.728 &  0.755 \\
                       & $CF_{ACC}$ $L_G$ &  0.347 &  0.368 &  0.419 &  0.432 &  0.473 &  0.580 &  0.626 &  0.685 &  0.736 \\ \midrule
$MGTCOM^{\mathcal{E}}$ 
                       & $LP_{ACC}$ &  0.702 &  0.778 &  0.851 &  0.876 &  0.919 &  0.936 &  0.958 &  0.972 &  0.963 \\
                       & $CF_{ACC}$ $L_y$ &  0.484 &  0.499 &  0.640 &  0.637 &  0.729 &  0.788 &  0.888 &  0.933 &  0.891 \\
                       & $CF_{ACC}$ $L_\mathcal{T}$ &  0.312 &  0.311 &  0.306 &  0.308 &  0.314 &  0.305 &  0.312 &  0.316 &  0.311 \\
                       & $CF_{ACC}$ $L_G$ &  0.382 &  0.412 &  0.479 &  0.491 &  0.555 &  0.600 &  0.665 &  0.721 &  0.706 \\ \midrule
$MGTCOM^{\mathcal{T}}$ 
                       & $LP_{ACC}$ &  0.636 &  0.678 &  0.669 &  0.639 &  0.671 &  0.653 &  0.644 &  0.671 &  0.638 \\
                       & $CF_{ACC}$ $L_y$ &  0.310 &  0.310 &  0.332 &  0.324 &  0.365 &  0.343 &  0.337 &  0.352 &  0.348 \\
                       & $CF_{ACC}$ $L_\mathcal{T}$ &  0.323 &  0.341 &  0.372 &  0.403 &  0.485 &  0.532 &  0.562 &  0.677 &  0.610 \\
                       & $CF_{ACC}$ $L_G$ &  0.227 &  0.228 &  0.248 &  0.242 &  0.248 &  0.237 &  0.225 &  0.234 &  0.221 \\
    \bottomrule
    \end{tabular}

% }
\end{table*}

==> figs/tab_parameters.tex <==
\begin{table}[ht!]
\centering
\caption{
    Parameter count comparison between node2vec and the $MGTCOM$ model.
    \label{tab:params}
}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{l|ll}
    \hline
    Dataset & node2vec  & $MGTCOM$  \\ \hline
    DBLP    & 683,968   & 173,910   \\
    ICEWS   & 669,632   & 1,072,302 \\
    IMDB    & 867,840   & 170,846   \\
    SDS     & 5,979,712 & 231,282   \\
    Cora    & 173,312   & 136,390   \\ \hline
\end{tabular}
% }
\end{table}

==> figs/tab_symbols.tex <==
\begin{table}[t]
\centering
\caption{
    Notation used in this paper.
    \label{tab:notation}
}
% \resizebox{\columnwidth}{!}{
\small
    \begin{tabular}{>{\centering\arraybackslash}m{2.1cm}|p{6cm}}
        \hline
        \textbf{Notation}           & \textbf{Description} \\ \hline
        $\mathcal{V}$               & The set of nodes in a graph                   \\ \hline
        $\mathcal{A}$               & The set of node types                         \\ \hline
        $\mathcal{E}$               & The set of edges in a graph                   \\ \hline
        $\mathcal{R}$               & The set of edge types/relations               \\ \hline
        $\mathcal{T}$               & The set of timestamps in a graph              \\ \hline
        $\mathcal{X}_{\phi(\cdot)}$ & Feature matrix for node type $\phi(\cdot)$    \\ \hline
        $\phi(v) \in \mathcal{A}$   & Type of node $v$                              \\ \hline
        $\psi(e) \in \mathcal{R}$   & Type of edge $e$                              \\ \hline
        $G_v$                       & $k$-hop neighborhood subgraph for node $v$    \\ \hline
        $d \in \mathbb{N}$          & Size of node embedding vector                 \\ \hline
        $E_v \in \mathbb{R}^d$      & Auxiliary embedding vector for node $v$       \\ \hline
        $Z_v \in \mathbb{R}^d$      & Primary embedding vector for node $v$         \\ \hline
        $Z_v^{\mathcal{E}}, Z_v^{\mathcal{T}} \in \mathbb{R}^d$ & Task specific embedding vectors for node $v$         \\ \hline
        $K \in \mathbb{N}$                                      & Number of communities                         \\ \hline
        $\mathcal{N}(\mu_k, \boldsymbol{\Sigma}_k), \theta_k$   & Parameters for the $k$'th cluster/community   \\ \hline
        ${\mu_k} \in \mathbb{R}^d$                              & $k$'th cluster mean vector                    \\ \hline
        $\boldsymbol{\Sigma}_k \in \mathbb{R}^{d\times d}$      & $k$'th cluster covariance vector              \\ \hline
        $\mathbf{z} \in \{0, .., K\}^{|\mathcal{V}|}$   & Community membership assignment vector        \\ \hline
        $\omega$                    & Interval window for temporal context sampling                     \\ \hline
        $P_l \in \mathcal{V}^l$     & Sampled context window of length $l$                              \\ \hline
        %                  &                      \\ \hline
    \end{tabular}
% }
\end{table}

==> front/acknow.tex <==
% \chapter*{Acknowledgements}

==> front/acronyms.tex <==
% \chapter*{Acronyms}

% \begin{acronym}[UML]
%   \acro{dem}[DEM]{digital elevation model}
%   \acro{dt}[DT]{Delaunay triangulation}
%   \acro{gdal}[GDAL]{Geospatial Data Abstraction Library}
%   \acro{gis}[GIS]{geographical information system}
%   \acro{giss}[GISs]{geographical information systems}
%   \acro{gui}[GUI]{graphical user interface}
%   \acro{tin}[TIN]{triangular irregular network}
%   \acro{vd}[VD]{Voronoi diagram}
% \end{acronym}

==> front/contents.tex <==

\setcounter{tocdepth}{2}

\tableofcontents
\listoffigures
\listoftables
\listofalgorithms



==> resources/figs/embed_ratio_tab.tex <==
\begin{tabular}{llllllllllllllll}
\toprule
                       & {} & \multicolumn{14}{l}{value} \\
                       & embed_node_ratio &           0.00 &           0.02 &           0.05 &           0.07 &           0.10 &           0.20 &           0.30 &           0.40 &           0.50 &           0.60 &           0.70 &           0.80 &           0.90 &           1.00 \\
model & variable &                &                &                &                &                &                &                &                &                &                &                &                &                &                \\
\midrule
$MGTCOM^{\mathcal{E}}$ & $CF_{ACC}$ $L_G$ &  0.556 ± 0.056 &  0.669 ± 0.021 &  0.662 ± 0.011 &  0.683 ± 0.011 &  0.691 ± 0.016 &  0.685 ± 0.022 &  0.677 ± 0.032 &  0.693 ± 0.017 &  0.669 ± 0.019 &  0.685 ± 0.047 &  0.679 ± 0.012 &  0.674 ± 0.032 &  0.675 ± 0.018 &  0.676 ± 0.023 \\
                       & $CF_{ACC}$ $L_\mathcal{T}$ &  0.317 ± 0.007 &  0.322 ± 0.006 &  0.313 ± 0.004 &  0.312 ± 0.003 &  0.315 ± 0.009 &  0.308 ± 0.002 &  0.313 ± 0.006 &  0.308 ± 0.007 &  0.311 ± 0.005 &  0.310 ± 0.007 &  0.309 ± 0.010 &  0.310 ± 0.001 &  0.304 ± 0.002 &  0.310 ± 0.008 \\
                       & $CF_{ACC}$ $L_y$ &  0.726 ± 0.041 &  0.886 ± 0.005 &  0.866 ± 0.016 &  0.893 ± 0.017 &  0.881 ± 0.009 &  0.854 ± 0.006 &  0.855 ± 0.026 &  0.871 ± 0.012 &  0.822 ± 0.002 &  0.853 ± 0.038 &  0.850 ± 0.009 &  0.825 ± 0.006 &  0.838 ± 0.007 &  0.846 ± 0.018 \\
                       & $LP_{ACC}$ &  0.774 ± 0.011 &  0.791 ± 0.006 &  0.791 ± 0.005 &  0.789 ± 0.010 &  0.792 ± 0.001 &  0.794 ± 0.003 &  0.787 ± 0.005 &  0.796 ± 0.007 &  0.793 ± 0.011 &  0.790 ± 0.014 &  0.794 ± 0.005 &  0.794 ± 0.005 &  0.783 ± 0.011 &  0.784 ± 0.006 \\
$MGTCOM^{\mathcal{T}}$ & $CF_{ACC}$ $L_G$ &  0.292 ± 0.025 &  0.355 ± 0.038 &  0.299 ± 0.053 &  0.313 ± 0.010 &  0.333 ± 0.020 &  0.314 ± 0.059 &  0.257 ± 0.020 &  0.264 ± 0.038 &  0.266 ± 0.052 &  0.242 ± 0.012 &  0.245 ± 0.043 &  0.260 ± 0.056 &  0.250 ± 0.043 &  0.228 ± 0.026 \\
                       & $CF_{ACC}$ $L_\mathcal{T}$ &  0.384 ± 0.061 &  0.344 ± 0.034 &  0.333 ± 0.013 &  0.338 ± 0.020 &  0.336 ± 0.013 &  0.333 ± 0.013 &  0.334 ± 0.019 &  0.338 ± 0.014 &  0.343 ± 0.038 &  0.569 ± 0.107 &  0.438 ± 0.160 &  0.481 ± 0.201 &  0.439 ± 0.152 &  0.536 ± 0.202 \\
                       & $CF_{ACC}$ $L_y$ &  0.451 ± 0.039 &  0.566 ± 0.057 &  0.474 ± 0.119 &  0.507 ± 0.033 &  0.535 ± 0.031 &  0.523 ± 0.123 &  0.408 ± 0.099 &  0.429 ± 0.048 &  0.427 ± 0.097 &  0.388 ± 0.014 &  0.384 ± 0.088 &  0.418 ± 0.099 &  0.378 ± 0.084 &  0.342 ± 0.046 \\
                       & $LP_{ACC}$ &  0.603 ± 0.071 &  0.624 ± 0.017 &  0.630 ± 0.019 &  0.630 ± 0.012 &  0.628 ± 0.022 &  0.632 ± 0.012 &  0.622 ± 0.004 &  0.630 ± 0.009 &  0.598 ± 0.073 &  0.627 ± 0.012 &  0.623 ± 0.018 &  0.618 ± 0.015 &  0.616 ± 0.015 &  0.618 ± 0.015 \\
\bottomrule
\end{tabular}


==> resources/figs/inference_tab.tex <==
\begin{tabular}{lllllllllll}
\toprule
                       & {} & \multicolumn{9}{l}{value} \\
                       & train_ratio &    0.1 &    0.2 &    0.3 &    0.4 &    0.5 &    0.6 &    0.7 &    0.8 &    0.9 \\
model & variable &        &        &        &        &        &        &        &        &        \\
\midrule
$MGTCOM$ & $CF_{ACC}$ $L_G$ &  0.347 &  0.368 &  0.419 &  0.432 &  0.473 &  0.580 &  0.626 &  0.685 &  0.736 \\
                       & $CF_{ACC}$ $L_\mathcal{T}$ &  0.323 &  0.333 &  0.370 &  0.408 &  0.483 &  0.566 &  0.664 &  0.728 &  0.755 \\
                       & $CF_{ACC}$ $L_y$ &  0.428 &  0.474 &  0.548 &  0.571 &  0.638 &  0.799 &  0.861 &  0.899 &  0.927 \\
                       & $LP_{ACC}$ &  0.686 &  0.728 &  0.774 &  0.755 &  0.780 &  0.833 &  0.861 &  0.887 &  0.872 \\
$MGTCOM^{\mathcal{E}}$ & $CF_{ACC}$ $L_G$ &  0.382 &  0.412 &  0.479 &  0.491 &  0.555 &  0.600 &  0.665 &  0.721 &  0.706 \\
                       & $CF_{ACC}$ $L_\mathcal{T}$ &  0.312 &  0.311 &  0.306 &  0.308 &  0.314 &  0.305 &  0.312 &  0.316 &  0.311 \\
                       & $CF_{ACC}$ $L_y$ &  0.484 &  0.499 &  0.640 &  0.637 &  0.729 &  0.788 &  0.888 &  0.933 &  0.891 \\
                       & $LP_{ACC}$ &  0.702 &  0.778 &  0.851 &  0.876 &  0.919 &  0.936 &  0.958 &  0.972 &  0.963 \\
$MGTCOM^{\mathcal{T}}$ & $CF_{ACC}$ $L_G$ &  0.227 &  0.228 &  0.248 &  0.242 &  0.248 &  0.237 &  0.225 &  0.234 &  0.221 \\
                       & $CF_{ACC}$ $L_\mathcal{T}$ &  0.323 &  0.341 &  0.372 &  0.403 &  0.485 &  0.532 &  0.562 &  0.677 &  0.610 \\
                       & $CF_{ACC}$ $L_y$ &  0.310 &  0.310 &  0.332 &  0.324 &  0.365 &  0.343 &  0.337 &  0.352 &  0.348 \\
                       & $LP_{ACC}$ &  0.636 &  0.678 &  0.669 &  0.639 &  0.671 &  0.653 &  0.644 &  0.671 &  0.638 \\
\bottomrule
\end{tabular}


==> resources/figs/performance.tex <==
\begin{tabular}{lllllllllll}
\toprule
    & model & GraphSAGE & Node2Vec &   ComE & GEMSEC &  CTDNE &  CP-GNN & $MGTCOM$ & $MGTCOM^{\mathcal{T}}$ & $MGTCOM^{\mathcal{E}}$ \\
dataset & variable &           &          &        &        &        &         &          &                        &                        \\
\midrule
Cora & $CF_{ACC}$ $L_\mathcal{T}$ &       nan &      nan &    nan &    nan &      - &     nan &        - &                      - &                    nan \\
    & $CF_{ACC}$ $L_y$ &     0.659 &    0.798 &  0.864 &  0.845 &      - &   0.780 &        - &                      - &                  0.854 \\
    & $COM_{NMI}$ $L_G$ &     0.507 &    0.543 &  0.635 &  0.632 &      - &   0.501 &        - &                      - &                  0.643 \\
    & $COM_{NMI}$ $L_\mathcal{T}$ &       nan &      nan &    nan &    nan &      - &     nan &        - &                      - &                    nan \\
    & $COM_{NMI}$ $L_y$ &     0.376 &    0.345 &  0.434 &  0.437 &      - &   0.370 &        - &                      - &                  0.439 \\
    & $LP_{ACC}$ &     0.505 &    0.939 &  0.962 &  0.923 &      - &   0.829 &        - &                      - &                  0.958 \\
    & Davies-Bouldin &     1.526 &    1.250 &  2.021 &  1.500 &      - &   2.634 &        - &                      - &                  2.647 \\
    & Modularity &     0.636 &    0.691 &  0.785 &  0.780 &      - &   0.677 &        - &                      - &                  0.754 \\
DBLPHCN & $CF_{ACC}$ $L_\mathcal{T}$ &     0.309 &    0.308 &  0.328 &  0.324 &  0.488 &   0.313 &    0.758 &                  0.373 &                  0.320 \\
    & $CF_{ACC}$ $L_y$ &     0.315 &    0.832 &  0.842 &  0.831 &  0.809 &   0.506 &    0.896 &                  0.508 &                  0.884 \\
    & $COM_{NMI}$ $L_G$ &     0.040 &    0.425 &  0.470 &  0.314 &  0.401 &   0.107 &    0.336 &                  0.028 &                  0.371 \\
    & $COM_{NMI}$ $L_\mathcal{T}$ &     0.006 &    0.033 &  0.025 &  0.022 &  0.059 &   0.022 &    0.209 &                  0.037 &                  0.026 \\
    & $COM_{NMI}$ $L_y$ &     0.051 &    0.549 &  0.463 &  0.385 &  0.537 &   0.209 &    0.465 &                  0.049 &                  0.492 \\
    & $LP_{ACC}$ &     0.624 &    0.710 &  0.735 &  0.544 &  0.701 &   0.522 &    0.743 &                  0.615 &                  0.794 \\
    & Davies-Bouldin &     0.472 &    2.305 &  2.205 &  4.056 &  1.206 &   4.780 &    2.039 &                  4.205 &                  5.188 \\
    & Modularity &     0.028 &    0.662 &  0.636 &  0.492 &  0.642 &  -0.035 &    0.427 &                  0.004 &                  0.514 \\
ICEWS & $CF_{ACC}$ $L_\mathcal{T}$ &     0.294 &    0.301 &  0.264 &  0.310 &  0.285 &   0.273 &    0.316 &                  0.319 &                  0.313 \\
    & $CF_{ACC}$ $L_y$ &       nan &      nan &    nan &    nan &    nan &     nan &      nan &                    nan &                    nan \\
    & $COM_{NMI}$ $L_G$ &     0.227 &    0.354 &  0.548 &  0.309 &  0.347 &   0.204 &    0.119 &                  0.001 &                  0.447 \\
    & $COM_{NMI}$ $L_\mathcal{T}$ &     0.018 &    0.040 &  0.015 &  0.022 &  0.022 &   0.013 &    0.057 &                  0.001 &                  0.011 \\
    & $COM_{NMI}$ $L_y$ &       nan &      nan &    nan &    nan &    nan &     nan &      nan &                    nan &                    nan \\
    & $LP_{ACC}$ &     0.525 &    0.936 &  0.880 &  0.768 &  0.921 &   0.709 &    0.903 &                  0.895 &                  0.945 \\
    & Davies-Bouldin &     1.027 &    1.697 &  2.559 &  3.867 &  1.533 &   4.737 &    3.883 &                  3.598 &                  3.182 \\
    & Modularity &     0.218 &    0.215 &  0.483 &  0.311 &  0.239 &   0.199 &    0.007 &                  0.001 &                  0.390 \\
IMDB & $CF_{ACC}$ $L_\mathcal{T}$ &     0.346 &    0.373 &  0.394 &  0.380 &  0.488 &   0.316 &    0.659 &                  0.556 &                  0.377 \\
    & $CF_{ACC}$ $L_y$ &       nan &      nan &    nan &    nan &    nan &     nan &      nan &                    nan &                    nan \\
    & $COM_{NMI}$ $L_G$ &     0.039 &    0.181 &  0.197 &  0.094 &  0.160 &   0.033 &    0.107 &                  0.031 &                  0.158 \\
    & $COM_{NMI}$ $L_\mathcal{T}$ &     0.022 &    0.025 &  0.031 &  0.013 &  0.065 &   0.004 &    0.239 &                  0.231 &                  0.026 \\
    & $COM_{NMI}$ $L_y$ &       nan &      nan &    nan &    nan &    nan &     nan &      nan &                    nan &                    nan \\
    & $LP_{ACC}$ &     0.714 &    0.757 &  0.666 &  0.637 &  0.728 &   0.598 &    0.721 &                  0.724 &                  0.773 \\
    & Davies-Bouldin &     0.301 &    1.803 &  3.840 &  4.951 &  1.749 &   4.806 &    2.257 &                  1.285 &                  4.013 \\
    & Modularity &    -0.172 &    0.190 &  0.395 &  0.073 &  0.196 &  -0.053 &    0.119 &                  0.114 &                  0.286 \\
SDS & $CF_{ACC}$ $L_\mathcal{T}$ &     0.521 &    0.445 &  0.386 &  0.384 &  0.447 &       - &    0.523 &                  0.887 &                  0.492 \\
    & $CF_{ACC}$ $L_y$ &       nan &      nan &    nan &    nan &    nan &       - &      nan &                    nan &                    nan \\
    & $COM_{NMI}$ $L_G$ &     0.186 &    0.277 &  0.346 &  0.117 &  0.233 &       - &    0.120 &                  0.043 &                  0.389 \\
    & $COM_{NMI}$ $L_\mathcal{T}$ &     0.250 &    0.149 &  0.117 &  0.015 &  0.161 &       - &    0.204 &                  0.536 &                  0.044 \\
    & $COM_{NMI}$ $L_y$ &       nan &      nan &    nan &    nan &    nan &       - &      nan &                    nan &                    nan \\
    & $LP_{ACC}$ &     0.922 &    0.953 &  0.758 &  0.878 &  0.955 &       - &    0.934 &                  0.616 &                  0.956 \\
    & Davies-Bouldin &     1.108 &    2.355 &  3.986 &  3.410 &  2.890 &       - &    2.474 &                  1.519 &                  2.559 \\
    & Modularity &     0.088 &    0.163 &  0.301 &  0.037 &  0.016 &       - &    0.015 &                  0.005 &                  0.374 \\
\bottomrule
\end{tabular}


==> settings.tex <==


\newcommand{\myName}{
    Egor Dmitriev (6100120) \\
    egordmitriev2@gmail.com
}
\newcommand{\myTitle}{MGTCOM: Community Detection in Temporal Multimodal Graphs}

\newcommand{\myUni}{Utrecht University}

\newcommand{\myGraduationYear}{2022}
\newcommand{\myGraduationMonth}{June}

\newcommand{\mySupervisorOne}{Dr. M. W. Chekol}
\newcommand{\mySupervisorTwo}{Dr. S. Wang}

%-- for names for \autoref commands
\def\chapterautorefname{Chapter}
\def\sectionautorefname{Section}
\def\subsectionautorefname{Section}
\def\subsubsectionautorefname{Section}
\def\algorithmautorefname{Algorithm}
 
%-- for pdf metadata
\hypersetup{pdfauthor={\myName}}
\hypersetup{pdfkeywords={community detection, representation learning, dynamic networks}}
\hypersetup{pdfsubject={A thesis submitted to the Utrecht University in partial fulfillment of the requirements for the degree of Master of Science in Computing Science}}
\hypersetup{pdftitle={\myTitle}}

%-- handy shortcuts
\newcommand{\ie}{i.e.}
\newcommand{\eg}{e.g.}

%-- colours for the hyperlinks
\definecolor{colorforlinks}{RGB}{27, 60, 131}



